Integrated cooling channels in position-sensitive silicon detectors

We present an approach to construct position-sensitive silicon detectors with an integrated cooling circuit. Tests on samples demonstrate that a very modest liquid flow very effectively cool the devices up to a power dissipation of over 10~W/cm$^2$. The liquid flow is found to have a negligible impact on the mechanical performance. A finite-element simulation predicts the cooling performance to an accuracy of approximately 10~\%.

==> conclusions.tex <==
- we have presented a low-pressure single phase MCC solution with in-plane connections

 - reliable connections to conventional circuit -> controlled measurements

 - very efficient cooling; up to 25 W/cm2 with minimal temperature increase (10ºC) in MCC region

 - thermal measurements are in good agreement with FE simulation

 - MCC minimal impact on mechanical stability 

 - Easy and robust assembly (3/3) with a 3D printed adaptor it is needed to optimize the glue quantity in order to low as maximum as possible the material budget and also to study differeents glues according with the boundary conditions of the experiment where the silicon staves are placed

 - MCC embedded in a Si sensor is a real option

